Model Predictive Control of Wind Turbines with Piecewise-Affine Power Coefficient Approximation

In this paper, an offset-free bilinear model predictive control approach for wind turbines is presented. State-of-the-art controllers employ different control loops for pitch angle and generator torque which switch depending on wind conditions. In contrast, the presented controller is based on one unified control law that works for all wind conditions. The inherent nonlinearity of wind turbines is addressed through a piecewise-affine approximation of the power coefficient, which is modelled in a mixed-integer fashion. The presented controller is compared to a state-of-the-art baseline controller in a numerical case study using OpenFAST. Simulation results show that the presented controller ensures accurate reference power tracking. Additionally, damage equivalent loads are reduced for higher wind speeds.

==> baselineController.tex <==
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8
% !TEX root = paper.tex

\section{BASELINE CONTROLLER}
\label{sec:baseline}

In this section, a state-of-the-art \ac{wt} controller \cite{Aho2012} is presented.
It serves as a baseline for comparison with the \ac{mpc} presented in \cref{sec:mpc}.
Generally, a \ac{wt} operates in four distinct regions, as depicted in \cref{fig:regions}.

\begin{figure}[htbp]
	\centering
	\input{figures/regionData}
	\caption{\acp{wt} operate in different regions depending on wind speed}
	\label{fig:regions}
\end{figure}

In Regions 1 and 4, when the wind speed is below $V_{cut-in}\in\Rp$ or above $V_{cut-out}\in\Rp$ the wind conditions do not allow a safe opration and no power is generated.
In Region 2, the available power 
\begin{equation}
	P_{r,max}(t) = m'V(t)^3\overline C_p\label{eq:availablePower}
\end{equation}
where $\overline C_p\in\Rp$ denotes the maximum power coefficient is below the desired power reference $P_e^t\in\Rp$. 
Therefore, the \ac{wt} is controlled such that $C_p$ and, consequently, the extracted power are maximized.
In Region 3, the wind speed surpasses $V_{th}(P_e^t)\in\Rp$ at which (\ref{eq:availablePower}) equals $P_e^t$.
Here, the available power is equal or above $P_e^t$ and the \ac{wt} is controlled such that generated power remains equal to $P_e^t$.
Two independent control loops are employed for generator torque and pitch angle which are presented in the following subsections.
Both, generator torque and pitch angle are computed based on low-pass filtered generator speed signals.
The low-pass filter function for the generator speed signal is defined as
\begin{align}
	\hat\omega_g(k) &= f_{lp}(\omega_g(k),\hat\omega_g(k-1),T_\alpha)\nonumber\\
	:=&\begin{cases}
		(1 - \frac{T_s}{T_\alpha-T_s})\omega_g(k) + \frac{T_s}{T_\alpha-T_s}\hat\omega_g(k-1) & \text{if } k>0\\
		\omega_g(0) & \text{otherwise},
	\end{cases}\label{eq:lpFilter}
\end{align}
where $T_\alpha>2T_s$ is a design parameter and $\hat\omega_g(k)\in\R$ is the filtered signal.
The \ac{blc}'s structure can bee seen in \cref{fig:baseLineDiagram}.
\begin{figure}[htbp]
	\centering
	\input{figures/baseLineDiagram}
	\caption{\ac{blc} structure}
	\label{fig:baseLineDiagram}
\end{figure}

\subsection{Torque Control}
\label{sec:ref_torque_control}
For torque control, the filtered generator speed $\hat\omega_M(k)\in\R$ according to
\begin{equation}
	\hat\omega_M(k) = f_{lp}(\omega_g(k),\hat\omega_M(k-1),T_M)
\end{equation}
is used.
The target generator torque is given by
\begin{equation}\label{eq:generatorTorqueCases}
	u_M^t(k) = \begin{cases}
		0, & \text{if } \hat\omega_M(k)\leq\omega_{12}\\
		c_{12}(\hat\omega_M(k) - \omega_{12}), & \text{if }\omega_{12}<\hat\omega_M(k)\leq\omega_2\\
		c_{2}\hat\omega_M(k)^2, & \text{if }\omega_2<\hat\omega_M(k)\leq\omega_g^t(k)\\
		P_e^t/\omega^t_g(k), & \text{if }\omega_g^t(k)<\hat\omega_M(k),
	\end{cases}
\end{equation}
where $\omega_{12},c_{12},\omega_2,c_2\in\Rp$ are design parameters.
$\omega^t_g(k)\in\R$ is given by
\begin{equation}
	\omega^t_g(k) = \min\left(\sqrt[3]{\frac{P^t_e(k)}{\eta c_2}},\omega_{g,N}\right),
\end{equation}
where $P^t_e(k),\omega_{g,N}\in\R$ denote the demanded power and rated generator speed, respectively.
$u_M^t(k)$ is first being saturated before being applied, i.e.
\begin{align}
u_M^{t,s}(k) &= \sat(u_M^t(k),\underline{u}_M,\overline{u}_M)\nonumber\\
&:=\begin{cases}
	\underline{u}_M, & \text{if } u_M^t(k)<\underline{u}_M\\
	\overline{u}_M, & \text{if } u_M^t(k)>\overline{u}_M\\
	u_M^t(k), & \text{otherwise}.
\end{cases}
\end{align}
Secondly,  the generator torque's rate of change 
\begin{equation}
\Delta u_M(k)=\frac{u_M^{t,s}(k) - u_M(k-1)}{T_S},
\end{equation}
is saturated by applying
\begin{equation}
\Delta u_M^s(k) = \sat(\Delta u_M(k),\Delta\underline{u}_M,\Delta\overline{u}_M).
\end{equation}
Since the generator's inverter dynamics are neglected,
\begin{equation}
	u_M^{t,s}(k) = u_M(k).
\end{equation}


\subsection{Pitch Control}
\label{sec:ref_pitch_control}
The target pitch angle $u_\theta^t(k)$ is computed using a PI control loop with gain scheduling based on the generator speed error $e(k)$,
\begin{equation}
e(k) = \hat\omega_\theta(k) - \omega^t_g(k),
\end{equation}
where the filtered generator speed for pitch control $\hat\omega_\theta(k)\in\R$ is given by
\begin{equation}
	\hat\omega_\theta(k) = f_{lp}(\omega_g(k),\hat\omega_\theta(k-1),T_\theta).
\end{equation}
In addition to the current speed error $e(k)$,  the previous errors are integrated,  i.e.
\begin{equation}
E(k) = \begin{cases}
	E(k-1)+T_s e(k),&\text{if }k>0\\
    u_\theta(0)/(K_IG_K(0)),&\text{otherwise},
\end{cases}
\end{equation}
where $E(k),K_I\in\R$ denote the integrated speed error and integral gain, respectively.
$G_K(k)\in\Rp$ denotes the gain scheduling factor
\begin{equation}
G_K(k)=\frac{1}{1+u_\theta(k-1)/K_K},
\end{equation}
where $K_K\in\Rp$ is a design parameter.
$E(k)$ is limited to $[\underline{E}(k),\overline{E}(k)]\subset\R$, i.e.
\begin{equation}
	E^s(k) = \sat(E(k),\underline{E}(k),\overline{E}(k)),
\end{equation}
where $\underline{E}(k)$ and $\overline{E}(k)$ are given by
\begin{equation}
	\underline{E}(k) = \frac{\underline{u_\theta}}{K_IG_K(k)},\qquad\overline{E}(k) = \frac{\overline{u_\theta}}{K_IG_K(k)}.
\end{equation}
The target pitch angle is then computed by,
\begin{equation}
u_\theta^t(k) = \big(K_P e(k) + K_I E^s(k)\big)G_K(k),
\end{equation}
where $K_P\in\R$ denotes the proportional gain.
Analogously to the torque control,  the pitch target angle is not directly applied to the plant.
It is ensured that $u_\theta^t(k)\in[\underline{u_\theta}, \overline{u_\theta}]$ and that the slew rate remains within $[\Delta\underline{u_\theta},\Delta\overline{u_\theta}]$, i.e.
\begin{align}
	u_\theta^{t,s}(k) &= \sat(u_\theta^t(k),\underline{u_\theta}, \overline{u_\theta})\\
	\Delta u_\theta^{t,s}(k) &= \sat(\Delta u_\theta^t(k),\Delta\underline{u_\theta},\Delta\overline{u_\theta}).
\end{align}
Since the pitch actuators' dynamics are neglected,
\begin{equation}
	u_\theta^{t,s}(k) = u_\theta(k).
\end{equation}


==> baselineControllerShort.tex <==
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8
% !TEX root = paper.tex

\section{BASELINE CONTROLLER}
\label{sec:baseline}

In this section, a state-of-the-art \ac{wt} controller \cite{Aho2012} is briefly explained.
For details, refer to \cite{Grapentin2022}.
It serves as a baseline for comparison with the \ac{mpc} presented in \cref{sec:mpc}.
Generally, a \ac{wt} operates in four distinct regions, as depicted in \cref{fig:regions}.

\begin{figure}[tb]
	\centering
	%\input{figures/regionData}
	\includegraphics{tikzPictures/regionData.pdf}
	\caption{\acp{wt} operate in different regions depending on wind speed.}
	\label{fig:regions}
\end{figure}

In Regions 1 and 4, when the wind speed is below $V_{cut-in}\in\Rp$ or above $V_{cut-out}\in\Rp$ the wind conditions do not allow a safe opration and no power is generated.
In Region 2, the available power 
\begin{equation}
	\overline P_r(k) = m'V(k)^3\overline C_p\label{eq:availablePower}
\end{equation}
where $\overline C_p\in\Rp$ denotes the maximum power coefficient is below the desired power $P_e^d\in\Rp$. 
Therefore, the \ac{wt} is controlled such that $C_p$ and, consequently, the extracted power are maximized.
In Region 3, the wind speed surpasses $V_{th}(P_e^d)\in\Rp$ at which (\ref{eq:availablePower}) equals $P_e^d$.
Here, the available power is equal or above $P_e^d$ and the \ac{wt} is controlled such that generated power remains equal to it.


The \ac{blc}'s structure is shown in \cref{fig:baseLineDiagram}.
\begin{figure}[b]
	\centering
	\input{figures/baseLineDiagram}
	%\includegraphics{tikzPictures/baseLineDiagram.pdf}
	\caption{Structure of baseline controller.}
	\label{fig:baseLineDiagram}
\end{figure}

